Site2Vec: a reference frame invariant algorithm for vector embedding of protein-ligand binding sites

Protein-ligand interactions are one of the fundamental types of molecular interactions in living systems. Ligands are small molecules that interact with protein molecules at specific regions on their surfaces called binding sites. Tasks such as assessment of protein functional similarity and detection of side effects of drugs need identification of similar binding sites of disparate proteins across diverse pathways. Machine learning methods for similarity assessment require feature descriptors of binding sites. Traditional methods based on hand engineered motifs and atomic configurations are not scalable across several thousands of sites. In this regard, deep neural network algorithms are now deployed which can capture very complex input feature space. However, one fundamental challenge in applying deep learning to structures of binding sites is the input representation and the reference frame. We report here a novel algorithm Site2Vec that derives reference frame invariant vector embedding of a protein-ligand binding site. The method is based on pairwise distances between representative points and chemical compositions in terms of constituent amino acids of a site. The vector embedding serves as a locality sensitive hash function for proximity queries and determining similar sites. The method has been the top performer with more than 95% quality scores in extensive benchmarking studies carried over 10 datasets and against 23 other site comparison methods. The algorithm serves for high throughput processing and has been evaluated for stability with respect to reference frame shifts, coordinate perturbations and residue mutations. We provide Site2Vec as a stand alone executable and a web service hosted at \url{http://services.iittp.ac.in/bioinfo/home}.

==> subsection/results/plic.tex <==
    \subsection{Benchmarking against DeepDrug3D on PLIC dataset}
        
        From the PLIC database \cite{anand2014plic}, five groups with more than three hundred binding sites have been extracted for this study.
        These groups are divided based on pocket shape and nature of residues.
        There is a total of 2,249 protein-ligand binding sites, and among these sites, 1507 sites are used to train the model that generates proper clusters and to train the auto-encoder as well.
        The rest of 742 pockets are treated as test data (test data size is $30\%$).
        \begin{table}[!h]
            \centering
            \caption{Performance analysis of \sitevec\ and Deepdrug3D to classify the binding sites on PLIC data set.}
            \begin{tabular}{@{}lll@{}}\toprule \textbf{Method} & \textbf{Accuracy} & \textbf{AUC} \\\midrule
                K-NN on Site2Vec & 0.97 & 0.990\\
                Decision tree on Site2Vec & 0.95 & 0.976 \\
                Random Forest on Site2Vec & \textbf{0.98} & \textbf{0.992}\\
                DeepDrug3D & 0.96 & 0.991 \\\bottomrule
            \end{tabular}
            \label{Tab:01} 
        \end{table}
        The quality of the vector embedding or fingerprint for a given binding site is evaluated using PLIC data set in this exercise.
        The vector representations of binding sites in the training data are fed to a classifier (Random Forest with 1000 trees).
        The performance of this method is measured by computing the ROC curve and deducing AUC score from the curve, described in section ~\ref{evlatech} .
        We report here an accuracy of 0.98 of \sitevec on PLIC data set.

        \begin{figure}[!t]
            \begin{center}
            \includegraphics[scale=0.5]{image/rocPlotPLCtogether.pdf}
            \caption{ROC plot for evaluating the proposed method and Deepdrug3D to classify the protein-ligand binding sites into five groups. The x-axis represents the False positive rate, and the y-axis denotes True positive rate.}
            \label{fig:rocProposedMethodPLIC}                
            \end{center}

        \end{figure} 
        

    
    
